Binary Fuse Filters: Fast and Smaller Than Xor Filters

Bloom and cuckoo filters provide fast approximate set membership while using little memory. Engineers use them to avoid expensive disk and network accesses. The recently introduced xor filters can be faster and smaller than Bloom and cuckoo filters. The xor filters are within 23% of the theoretical lower bound in storage as opposed to 44% for Bloom filters. Inspired by Dietzfelbinger and Walzer, we build probabilistic filters -- called binary fuse filters -- that are within 13% of the storage lower bound -- without sacrificing query speed. As an additional benefit, the construction of the new binary fuse filters can be more than twice as fast as the construction of xor filters. By slightly sacrificing query speed, we further reduce storage to within 8% of the lower bound. We compare the performance against a wide range of competitive alternatives such as Bloom filters, blocked Bloom filters, vector quotient filters, cuckoo filters, and the recent ribbon filters. Our experiments suggest that binary fuse filters are superior to xor filters.

==> garbage.tex <==


\newpage

set member
There are many ways to construct a probabilistic filter that never fails to indicate set membership, but that 

In practice, all 

A \emph{Bloom filter} works
on 

consist of a collection of  hash functions $h_1$, $h_2$, \ldots, $h_k$, which map each possible key to a fixed integer which we interpret as an index value, and an array of bits $B$, initialized with zeros. The size of the array and the number of hash functions $k$ are parameters of the filter.
When we add a key $x$, we hash it with each hash function, and set the corresponding bits: \begin{eqnarray*}B[{h_1(x)}] & \leftarrow 1,\\ B[{h_2(x)}] & \leftarrow 1,\\ & \vdots \\ B[{h_k(x)}] & \leftarrow 1.\end{eqnarray*} To determine whether a given key is likely present, we check that the corresponding bits in our array are set: \begin{eqnarray*}(B[{h_1(x)}] = 1) \mathrm{~and~} (B[{h_2(x)}] = 1) \mathrm{~and~} \cdots \mathrm{~and~} (B[{h_k(x)}] = 1).\end{eqnarray*}
 Thus, if there are $k$~hash functions, we might need to check up to $k$~bits. For keys that were added, we are guaranteed that all bits are set: there can never be a false negative. But false positives are possible, if the bits were set by other keys. The standard Bloom filter does not allow us to remove keys.
Bloom filters  support adding keys irrespective of the size of the bit array and of
%the number of hash functions, but the false-positive probability increases as $2^{\frac{M}{2 N}}$
%given an initial capacity $M$ and a key count $N$.
the number of hash functions, but the false-positive probability increases as more entries are added, and so more bits are set.
%\hl{Thomas: I don't quite understand what "increases as" means... Is it correct? Or should it be "increases at"? Also I'm afraid I didn't find this formula... According to e.g. Wikipedia, the exact formula of false positives is quite complex... Maybe we omit the formula here? I rewrote this (original is commented).}


The size of the array $B$ is typically chosen so that a certain false-positive probability can be guaranteed up to a maximal number of entries, and the  optimal parameter $k$ is calculated. %If chosen well, about half of the bits in the array are set.
The expected space overhead for optimal Bloom filters is 44\%: it requires setting $k = - \log_2 \epsilon$ where $\epsilon$ is the desired bound on the false-positive probability. %Each addition and membership test needs $k$~memory accesses. 
Bloom filters can be made concurrent~\cite{5476244}.

\emph{Blocked Bloom filters}~\cite{Putze:2010:CHS:1498698.1594230,lang2019performance} consist of many small Bloom filters, maybe one per CPU cache line, so that they need only one memory access per operation. However, the load of those small filters is likely to be uneven, and so for the same false-positive probability, they often need about 30\% more space than standard Bloom filters. Advanced CPU instructions allow to speed up membership tests for both regular and blocked Bloom filters~\cite{Polychroniou:2014:VBF:2619228.2619234}.

There are many other variations on Bloom filters including counting Bloom filters~\cite{Bonomi:2006:ICC:1276191.1276252,Rottenstreich:2014:VCB:2736196.2736202} which support removing keys at the expense of more storage, compressed Bloom filters~\cite{Mitzenmacher:2002:CBF:581876.581878}, multidimensional Bloom filters~\cite{Crainiceanu:2015:BLO:2825276.2825463}, Stable Bloom filters~\cite{Deng:2006:ADD:1142473.1142477} and so forth.

\subsection{Fingerprint Based Variants}
Fingerprint-based variants store a fingerprint per key, where a fingerprint is  the result of  hash function $h$; typically, it is a word having a fixed number of bits. The membership test  consists of the retrieval and comparison  with the relevant fingerprints for the given key.
The general intuition is as follows. For each value $x$ in the set, we store the fingerprint $h(x)$ in a key-fingerprint data structure. %We require that if we later attempt to access the fingerprint for $x$ from the data structure, we always get $h(x)$. 
Given a candidate value $y$, we access its fingerprint from the data structure and we compare the result with $h(y)$. Whenever $y$ was part of the set, the fingerprints match, otherwise they are likely different with a probability that depends on the size of the fingerprint.

\begin{itemize}
\item \emph{Golomb-compressed sequences}~\cite{Putze:2010:CHS:1498698.1594230} store the sorted fingerprints by encoding the differences between fingerprint values. The overhead of this encoding is at least 1.5~bits per key, but it is difficult to achieve competitive  speed. %, and so we did not include them in our performance plots.

\item \emph{Cuckoo filters}~\cite{Fan:2014:CFP:2674005.2674994} are based on cuckoo hashing. At full capacity, and with a low false-positive probability, they use less space than Bloom filters, and membership tests are often faster. The overhead is 3~bits per key for the standard cuckoo filter, and 2~bits per key for the slower semi-sorted variant.  We are not aware of a cuckoo filter implementation that supports concurrent updates though there are  related cuckoo hashing concurrency strategies~\cite{Li:2014:AIF:2592798.2592820}.

\item \emph{Quotient filters}~\cite{Pandey:2017:GCF:3035918.3035963} store fingerprints in a compact hash table. Quotient filters and cuckoo filters use a similar amount of memory.

\item \emph{Morton filters}~\cite{Breslow:2018:MFF:3213880.3232248} are similar to cuckoo filters, but use underloaded buckets, like Horton tables~\cite{Breslow:2016:HTF:3026959.3026986}.
%This ensures that most entries can be stored in the first bucket. 
Many sparse buckets are combined into a block so that data is stored more densely. 
%Morton filters require highly optimized code in order to perform well, so we were hoping we can use the implementation of the original authors. Unfortunately, we did not get the source code in time in order to evaluate them thoroughly. From what we understand, to be faster than cuckoo filters, lookups need to be batched, which is only possible for some use cases.

\item \emph{Bloomier filters}~\cite{Chazelle:2004:BFE:982792.982797, charles2008bloomier} support approximate evaluation of arbitrary functions, in addition to approximate membership queries. 
We are interested in a  variant of the Bloomier filter~\cite{10.1007/978-3-540-70575-8_32}
that can be used for approximate membership queries. We call this variant the xor filter (\S~\ref{xor}).




\end{itemize}
%%%%%%%% Simplifying
Other variants have been proposed~\cite{10.1007/978-3-642-03351-3_25,10.1007/978-3-319-94144-8_24} but authors sometimes omit to provide and benchmark practical implementations.
Dietzfelbinger and Pagh~\cite{10.1007/978-3-540-70575-8_32} observe that fingerprint techniques can be extended by storing auxiliary data with the fingerprint.

\newpage
Rest is garbage at this point


For rare events: It is also possible to use layers of filters. So you start with Xor8, but instead of falling back entirely, you fall back on a second xor8 filter with an independent seed. Since the bulk of the pressure is on the first filter, it tends to stay in cache while the second filter remains cold but still faster than a full lookup. This scales to as many filters as you'd like.

Go implementation might prove to be an additional validation.

For batch filtering queries, it might be possible to exploit the locality of binary fuse filters to improve the performance.


----

explain the better construction performance (better locality, prefetch for the first part, scan twice)

probability of mapping step; small sets (less than 1 million keys)

test with huge pages

explain the name "binary fuse filter" means the segment length is a power of two.
explain why this is fine, and why it is faster / how much faster.

----

Practically, Bloom filters are often slower and larger than alternatives such as cuckoo filters~\cite{Fan:2014:CFP:2674005.2674994}. 
Can we do better than even cuckoo filters?
%We compare various filter implementations in terms of performance, space usage, and features.

%\hl{This story now seems wrong:}
Bonomi et al.~\cite{Bonomi:2006:ICC:1276191.1276252} as well as Broder and Mitzenmacher~\cite{broder2004network} remarked that
for static sets, essentially optimal memory usage is possible using a \emph{perfect hash function} and fingerprints. 
They dismissed this possibility in part %because it does not allow for changes in the set, and 
because perfect hash functions might be too expensive to compute. 
Yet Dietzfelbinger and Pagh~\cite{10.1007/978-3-540-70575-8_32} described a seemingly practical implementation
of this idea which we call an xor filter. It builds on closely related work such as Bloomier filters~\cite{Chazelle:2004:BFE:982792.982797, charles2008bloomier}. %Dietzfelbinger and Pagh used it as a secondary data structure in a theoretical construction. 



The high speed of the construction of binary fuse filters has to do with how inexpensive the hashing function is, but also they have to do with locality. See whyfaster.txt, make plot.


In the experimental section, explain how we design the benchmark so to avoid inlining, report how we got it wrong with respect to in/out mixing in our earlier paper.

Can we go 32-bit?

Discuss how we can always go very low if we are willing to sacrifice build times.


we use splitmix throughout.

%However,
\section{Xor Filters}
\label{xor}

%\subsection{Overview}

Given a key $x$, we produce its
$k$-bit fingerprint (noted $\fingerprint(x)$) using a randomly chosen hash function. We assume an idealized fully independent hash function; all fingerprints are equally likely so that  $P(\fingerprint(x) = c) =  1/2^k$ for any $x$ and $c$. 
%\hl{Thomas: is it really smaller equal? I think it is just equal... the fingerprint is n bit, and comparing it against a random n-bit value can not have a smaller probability... I think.}
This probability $\epsilon = 1/2^k$ determines the false-positive probability of our filter. 
We summarize our notation in Table~\ref{table:notation}. 
% \hl{We used to require the fingerprint to come from a fully independent hash function, but I think that it is more than what we need. We only care about pairwise collisions, so universal is enough, and universality is easy (whereas full independence is impractical).}

% Thomas: I originally wrote this in the construction algorithm, as follows:

% Like the cuckoo filter and similar algorithms, we use fingerprints of the keys in the set, where a fingerprint is a number of bits of the hash of the key. The larger the fingerprint, the lower the false-positive rate of the filter. We store the fingerprint data in a table $B$ for later lookup.

% Unlike the cuckoo filter and similar algorithms, we don't store each fingerprint in its own dedicated cell, but only such that allows us to compute the fingerprint of a given key, from three cells. This allows the lookup algorithm to compare the stored fingerprint with the fingerprint of the requested key.

% The xor filter is similar to the BDZ perfect hash function~\cite{Botelho:2007:SSM:2394893.2394911}, except that we store data to reconstruct fingerprints, instead of data to construct a perfect hash function. Also related is the Bloomier filter~\cite{Chazelle:2004:BFE:982792.982797}, which stores indices.

%We begin by illustrating xor filters with an example, before giving a formal description.
We want to construct a map $F$ from all possible elements to
$k$-bit integers such that it maps all keys $y$
from a set $S$ to their $k$-bit  $\fingerprint(x)$.
Thus, if we pick any element of the set, it
gets mapped to its fingerprint by design $F(y)=\fingerprint(y)$. Any value that is not
part of the filter  gets mapped to a value distinct from its fingerprint
with a probability $1-\epsilon = 1- 1/2^k$.

We store the fingerprints in an array $B$ with capacity $c$ slightly larger than
the cardinality of the set $|S|$ (i.e., $c \approx 1.23 \times |S|$).
We randomly and independently choose
three hash functions
$h_0, h_1, h_2$ from $U$ to consecutive ranges of integer
values ($h_0: S \to \{0,\ldots, c/3 - 1\} $, $h_1: S \to \{c/3,\ldots,2c/3 - 1\} $, $h_2: S \to \{2c/3,\ldots,c-1\} $).
For example, if $c=12$, we might have the ranges $\{0,\ldots, 3\}$,
$\{4,\ldots, 7\}$, and
$\{8,\ldots,11\}$.
Our goal is to have that the exclusive-or aggregate of the values in array $B$ at
the locations given by the three hash functions agree with the fingerprint ($B[{h_0(x)}] \xor B[{h_1(x)}] \xor B[{h_2(x)}] = \fingerprint(x)$) for all elements $x \in S$. The hash functions $h_0, h_1, h_2$ are assumed to  be  independent from the hash function used for the fingerprint. 
%\hl{I have added this last sentence. 
%You want $P(\fingerprint(x) = f_1 \land h_k(x) = y_k) = P(\fingerprint(x) = f_1) \times P(h_k(x)  = y_k ) $ otherwise bad things may happen to you and your family.
%Thomas: I agree, I noticed fpp was sometimes slightly bad when I used fingerprint=hash. Now the implementation uses $hash \xor (hash >> 32)$, 
%and that effect disappeared. I will change it again as soon as I see any symptoms in my family.
%}

\begin{table}
\caption{Notation\label{table:notation}
}
\centering
\begin{tabular}{cp{10cm}}\toprule
$U$ & universe of all possible elements (e.g., all strings) \\
 $S$ & a set of elements from universe $U$ (also called ``keys'') \\
  $|S|$ & cardinality of the set $S$ \\
  $B$ & array of $k$-bit values \\
  $c=|B|$ & size (or capacity) of the array $B$, we set $c = \lfloor 1.23 \cdot |S| \rfloor + 32$  \\ 
  $\fingerprint$ & random hash function mapping elements of $U$ to $k$-bit values (integers in  $[0,2^k)$) \\
 $h_0, h_1, h_2$ & hash functions from $U$ to  integers in $[0,\lfloor c/3\rfloor)$,  $[\lfloor c/3\rfloor,\lfloor 2c/3\rfloor)$, $[\lfloor 2c/3 \rfloor,c)$
 respectively  \\
 %$\seed{}$ & seed value defining the hash functions  $h_0, h_1, h_2$ \\
 $x \xor y $ & bitwise exclusive-or between two values \\
 $B[i]$ & the $k$-bit values at index $i$ (indexes start at zero) \\
$\epsilon$ & false-positive probability \\
\bottomrule
\end{tabular}
\end{table}

%    Let $c=\lfloor 1.23 \cdot |S| + 32\rfloor/3$. \\ We require that
%    \begin{itemize}
%   \item $h_0: \{0,1,\ldots,2^k-1\} \to [0,\lfloor c/3\rfloor)$,
%   \item $h_1: \{0,1,\ldots,2^k-1\} \to  [\lfloor c/3\rfloor,\lfloor 2c/3\rfloor)$,
%   \item $h_2:\{0,1,\ldots,2^k-1\}  \to [\lfloor 2c/3 \rfloor,c)$,
%    \end{itemize}

\subsection{Membership Tests}
The membership-test function (Algorithm~\ref{alg:lookup}) calculates the hash functions $h_0, h_1, h_2$, then constructs the expected fingerprint from those entries in table $B$, and compares it against the fingerprint of the given key. If the key is in the set, the table  contains the fingerprint and so it matches. %If the key is not in the set, the fingerprint only matches with a probability of $1/2^k$, where $k$ is the number of bits in the fingerprint. 

The processing time includes the computation of three hash functions as well as three random memory accesses. Though other related
data structures may need fewer memory accesses, 
most modern processors can issue more than three memory accesses concurrently thanks to memory-level parallelism~\cite{jonathan2018exploiting, psaropoulos2017interleaving,akram2016boosting}. Hence, we should not expect the processing time to increase directly with the number of memory accesses. 
%Furthermore, the membership-test function of xor filters is essentially branch-free: there are no mispredicted branches. %Having fewer difficult-to-predict branches is often beneficial to performance on current processors due to pipelining and superscalar execution. 
% \hl{Cutting things short here since we repeat some of it later.}

\begin{algorithm}
\caption{Membership test\label{alg:lookup}: returns true if the key $x$ is likely in $S$, false otherwise}
\begin{algorithmic} % enter the algorithmic environment
    \REQUIRE key $x \in U$
   % \STATE $x \leftarrow \hash((k, \seed{})$
    \STATE \textbf{return} $\fingerprint(x) = B[h_0(x)] \xor B[h_1(x)] \xor B[h_2(x)]$
\end{algorithmic}
\end{algorithm}

\subsection{Construction}


%An $r$-partite hypergraph is a generalization of an undirected graph where each edge connects $r \geq 2$ vertices (nodes). Like Belazzougui et al.~\cite{Botelho:2007:SSM:2394893.2394911}, we first construct a 3-partite hypergraph from $S$, as it needs the least space. Then we fill in the fingerprint data into the table $B$ in the right order, so that the lookup algorithm can reconstruct them as needed. This requires  the table $B$ to be at least 23\% larger than the number of keys for the algorithm to work with high probability. This also implies that $0.23/1.23 \approx 0.19$ of the cells are unused. If construction fails, we try again with  new hash functions.


%\subsubsection{Mapping Step}

 
The construction follows the algorithm from Botelho et al.~\cite{Botelho:2007:SSM:2394893.2394911} to build acyclic 3-partite random hypergraphs. We apply Algorithm~\ref{alg:construct} which calls Algorithm~\ref{alg:mapping} one or more times until it succeeds,
passing randomly chosen hash functions $h_0, h_1, h_2$ with each call. 
In practice, we pick hash functions by generating
a new pseudo-random \emph{seed}. 
Finally, we apply Algorithm~\ref{alg:assigning}.

\begin{algorithm}
  \caption{Construction\label{alg:construct}}
  \begin{algorithmic}
      \REQUIRE set of keys $S$
      \REQUIRE a $\fingerprint$ function
      \REPEAT
          \STATE pick three hash functions $h_0, h_1, h_2$ at random, independently from the $\fingerprint$ function
      \UNTIL{$\map(S, h_0, h_1, h_2)$ returns success with a stack  $\stack{}$ (see Algorithm~\ref{alg:mapping})}
      \STATE $B \leftarrow$ an array of size $\lfloor 1.23 \cdot |S| \rfloor + 32$ containing $k$-bit values (uninitialized)
      \STATE $\assign(\stack{}, B, h_0, h_1, h_2)$ (see Algorithm~\ref{alg:assigning})
      \STATE \textbf{return} the array $B$ and the hash functions  $h_0, h_1, h_2$
  
  \end{algorithmic}
  \end{algorithm}
  

Algorithm~\ref{alg:mapping} works as follows. We initialize a (temporary) array $H$ of sets of keys of size  $\lfloor 1.23 \cdot |S| \rfloor + 32$.
At the beginning, all sets are empty. Then we take each key $x$ from the set $S$, and we hash it three times ($h_0(x), h_1(x), h_2(x)$).
We append the key $x$ to the three sets indicated by the three hash values (sets $H[h_0(x)], H[h_1(x)], H[h_2(x)]$).
Most sets in the table $H$  contain multiple keys, but almost surely some  contain exactly one key. 
We keep track of the sets containing just one key.
Repeatedly, we pick one such location, append it to the output stack together with the key $x$ it contains; 
each time we remove the key  $x$ from its three locations ($h_0(x), h_1(x), h_2(x)$).
The process either terminates with a stack containing all of the keys in which case we have a success, or with a failure.

The probability of success approaches 100\% if the set is large~\cite{Molloy:2005:CRH:1072778.1072783}.
For sets of size $10^7$,  Botelho et al.~\cite{Botelho:2007:SSM:2394893.2394911} found that the probability is almost 1.  For smaller sets, we experimentally found  that the estimated probability is always greater than $0.8$ with $c = 1.23 \cdot |S| + 32$, as shown in Fig.~\ref{fig:probMappingStep}.


Algorithm~\ref{alg:mapping} runs in linear time with respect to the size of the input set $S$ as long as adding and removing
a key $x$ from a set in $H$ is done in constant time. Indeed, each key $x$ of $S$ is initially added to three sets in $H$
and removed at most once from the same three sets.

In practice, if the keys in $S$ are integer values or other fixed-length objects, we can implement the  sets  using 
an integer-value counter and a fixed-length mask  (both initialized with zeros). When adding a key, we increment the counter and
compute the exclusive-or of the key with the mask, storing the result as the new mask. We similarly remove a key by decrementing
the counter and computing the same exclusive-or. 
Even when the set is made of large or variable-length elements, it may still be practical to represent them as small fixed-length (e.g., 64-bit or 128-bit) integers by hashing: it only comes at the cost of introducing a small error when two hash values collide, an improbable event that may only minutely increase the false-probability probability.


\begin{figure}\centering
\begin{tikzpicture}
\begin{axis}[
      xlabel={set size, $|S|$},
      ylabel={mapping step success probability},
      xmode=log,
      ymin = 0.4,
      legend pos=south east
      ]
\addplot[mark=triangle*, color=red] table {
3 0.986
9 0.949
27 0.865
81 0.853
243 0.767
729 0.733
2187 0.712
6561 0.815
19683 0.926
59049 0.997
177147 1.0
531441 1.0
};
\addlegendentry{$|B| = 1.23 \cdot |S| + 16$}
\addplot[mark=*, color=blue] table {
3 0.994
9 0.986
27 0.965
81 0.944
243 0.959
729 0.9
2187 0.848
6561 0.862
19683 0.948
59049 0.999
177147 1.0
531441 1.0
};
\addlegendentry{$|B| = 1.23 \cdot |S| + 32$}
\addplot[mark=square*, color=green] table {
3 1.0
9 0.998
27 0.989
81 0.979
243 0.983
729 0.986
2187 0.978
6561 0.953
19683 0.975
59049 0.999
177147 1.0
531441 1.0
};
\addlegendentry{$|B| = 1.23 \cdot |S| + 64$}
\end{axis}
\end{tikzpicture}
  \caption{Probability of mapping step, found experimentally with 1000 randomly generated sets.}
  \label{fig:probMappingStep}
\end{figure}


\begin{algorithm}
\caption{Mapping Step\label{alg:mapping} ($\map$)}
\begin{algorithmic}
    \REQUIRE set of keys $S$, $k$-bit integer-valued hash functions $h_0, h_1, h_2$.
    \STATE let $c \leftarrow \lfloor 1.23 \cdot |S| \rfloor + 32$
%    Let $c=\lfloor 1.23 \cdot |S| + 32\rfloor/3$. \\ We require that
%    \begin{itemize}
%   \item $h_0: \{0,1,\ldots,2^k-1\} \to [0,\lfloor c/3\rfloor)$,
%   \item $h_1: \{0,1,\ldots,2^k-1\} \to  [\lfloor c/3\rfloor,\lfloor 2c/3\rfloor)$,
%   \item $h_2:\{0,1,\ldots,2^k-1\}  \to [\lfloor 2c/3 \rfloor,c)$,
%    \end{itemize}
%    \STATE $C \leftarrow$ an array of size $c$ containing counters (initialized with zeros)
    \STATE $H \leftarrow$ an array of size $c$ containing a set of keys (values from $S$), initially empty
    
    \FORALL{$x$ in $S$}
    %    \FOR{$j=0$ \TO 2}
%            \STATE $C[h_{0}(x)] \leftarrow C[h_{0}(x)] + 1$
            \STATE append $x$ to $H[h_{0}(x)]$
 %           \STATE $C[h_{1}(x) ] \leftarrow C[h_{1}(x)] + 1$
            \STATE append $x$  to $H[h_{1}(x) ]$
  %          \STATE $C[h_{2}(x)] \leftarrow C[h_{2}(x)] + 1$
            \STATE append $x$ to $H[h_{2}(x)]$
            %   \ENDFOR
    \ENDFOR
    \STATE $Q\leftarrow$ initially empty queue
    \FOR{$i=0$ \textbf{to} $|H|$}
        \STATE \textbf{if} the set $H[i]$ contains a single key \textbf{then} add $i$ to $Q$ \textbf{endif}
    \ENDFOR
    \STATE $\stack{} \leftarrow$ initially empty stack
    \WHILE{queue $Q$ is not empty}
        \STATE remove an element $i$ from the queue $Q$
        \IF {the set $H[i]$ contains a single key}
            \STATE let $x$ be the sole value in the set $H[i]$
            \STATE push the pair $(x,i)$ on the stack $\stack{}$
            \FOR{$j=0$ \TO 2}
%                \STATE $C[h_{j}(x)] \leftarrow C[h_{j}(x)] - 1$
                \STATE remove $x$ from the set $H[h_{j}(x)]$
                \STATE \textbf{if} the set $H[h_{j}(x)]$ contains a single key  \textbf{then} add $h_{j}(x)$ to $Q$ \textbf{endif}
            \ENDFOR
        \ENDIF
    \ENDWHILE
    \STATE \textbf{return} success and the stack $\stack{}$ \textbf{if} $|\stack{}| = |S|$, \textbf{else} return failure
\end{algorithmic}
\end{algorithm}

%\subsubsection{Assigning Step}
We find it interesting to consider the second part of 
Algorithm~\ref{alg:mapping} when it succeeds. We iteratively 
empty the queue $Q$, one element at a time.
At iteration $t$, we add the key $x$ and the corresponding 
index $i$  to the stack if $x$ is the single key of set $H[i]$, and
we remove the key $x$ from the sets at 
locations $h_0(x), h_1(x), h_2(x)$.
Hence,  by construction, each time Algorithm~\ref{alg:mapping} 
adds a key $x$ and an index $i$ to the stack, the index $i$ is 
different from indexes $h_0(x'), h_1(x'), h_2(x')$ for 
all keys $x'$ encountered later (at time $t'>t$).

To construct the xor filter, we allocate an array $B$ large enough to store $\lfloor 1.23 \cdot |S| \rfloor + 32$ fingerprints.
We iterate over the keys and their indexes in the reverse order, compared to how they were identified  in the ``Mapping Step'' (Algorithm~\ref{alg:mapping}). 
For each key, there are three corresponding locations $h_0(x), h_1(x), h_2(x)$ in the table $B$; the index associated with the key
is one of $h_0(x), h_1(x), h_2(x)$. We set the value of $B[i]$ so that 
$B[h_0(x)] \xor B[h_1(x)] \xor B[h_2(x)] = \fingerprint(x)$.
%we set the entry in the table $B$ to the fingerprint of the key, xor $B[\mathrm{second~location}]$, xor $B[\mathrm{third~location}]$.
We repeat this for each key. Each key is processed once. 


By our construction, an entry in $B$ is modified at most once. After we modify an entry  
$B[i]$, then none of the values $B[h_0(x)]$, $B[h_1(x)]$, $B[h_2(x)]$ will ever be modified again.
This follows by our argument where we work through  Algorithm~\ref{alg:mapping} in reverse: 
$i$ is different from $h_0(x'), h_1(x'), h_2(x')$ for all keys $x'$ encountered so far. Remember that we use a stack, so the last entry added to the stack in Algorithm~\ref{alg:mapping} is removed first in Algorithm~\ref{alg:assigning}.
Thus, our construction is correct: we have that
\begin{align*}B[h_0(x)] \xor B[h_1(x)] \xor B[h_2(x)] = \fingerprint(x)\end{align*} for all keys $x$ in $S$ at the end of Algorithm~\ref{alg:assigning}.

\begin{algorithm}
\caption{Assigning Step\label{alg:assigning} ($\assign$)}
\begin{algorithmic}
    \REQUIRE $\stack{}$, target array for fingerprint data $B$, hash functions $h_0, h_1, h_2$
    \FOR{$(x,i)$ in  stack $\stack{}$}
    \STATE $B[i] \leftarrow 0$
    \STATE $B[i] \leftarrow \fingerprint(x) \xor B[h_0(x)] \xor B[h_1(x)] \xor B[h_2(x)]$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

%\subsection{Xor Filter Variants}


%\begin{itemize}
%\item A Bloom filter lookup of a key in the filter (a match) requires $O(k)$ memory accesses, where $k$ depends on the false-positive rate, so more accurate filters are slower. For keys not in the filter, on average 2 memory accesses are needed. Adding more entries than the capacity is possible but increases the false-positive rate.
%\item The blocked Bloom filter only requires one memory access per lookup in all cases, but needs more space than a Bloom filter.
%\item The cuckoo filter needs at most two memory accesses per lookup. Adding entries is allowed within the capacity.
%\item The counting quotient filter and the Morton filter on average need slightly more than one memory access per lookup. Adding entries is also allowed within the capacity.
%\item The Golomb-compressed sequence uses variable-bit-length codes, which slows down lookup. They are typically immutable.
%\end{itemize}


\subsection{Space Optimization: Xor+ Filter}
\label{sec:xorplus}

About 19\% of the entries in table $B$ are empty: for each 100~keys, we need 123~entries, and 23~are empty. 
%\hl{Thomas: "for 100~keys, we need 123~entries" is quite true due to using +32 entries... so I changed it to "for each 100 keys,..."}
For transmission, much of this empty space can be saved as follows:
before sending $B$, send a bit array that contains '0' for empty entries
and '1' for occupied entries. Then we only send the data of the occupied entries.
If we use $k=8$~bits, the regular xor filter needs $8 \times 1.23 = 9.84$~bits per entry, 
which we can compress in this way to $ 8 + 1.23 = 9.23$~bits per entry. 
%Filters with a low false-positive rate  benefit most from this optimization.
If space usage at runtime is more important than query speed, compression can be used at runtime. 
We can get a constant time access using a rank data structure such as Rank9~\cite{vigna2008broadword}, at the expense of a  small storage overhead ($\approx$25\%), or poppy~\cite{zhou2013space} for an even smaller overhead ($\approx$3\%) at the expense of some speed. %\hl{We apparently happy with the $\approx$25\% overhead of Rank9 and uninterested in poppy. I think that there are even better alternatives than poppy these days. Thomas: I didn't know about poppy. It looks like it could save 1\% space, at the cost of some speed. I will investigate a bit. (I think poppy is slower than rank9... at least it looks slower, having a loop.)}  

By changing the construction algorithm slightly, we can move most of the empty entries to the last third of the table $B$. To do so, we change the mapping algorithm so that three queues are used instead of one: one for each hash function---each hash function represents a third of the table $B$. We then process entries of the first two queues until those are empty, before we process entries from the third queue. 
Experimentally, we find that 36\% of the entries in the last third of  table $B$ are empty on average. If the rank data structure is then only constructed for this part of the table, space can be saved without affecting the membership-test performance as much, as only one rank operation is needed. 
We refer to this algorithm as ``xor+ filter'', using Rank9 as the default rank data structure. %\hl{We need to be explicit that we rely on Rank9, as there are smaller and more faster alternatives. Like poppy.} 
With the fingerprint size in bits $k$, it needs 
$k \times 1.23 \times 2/3$ bits per key for the first two thirds of the table $B$, 
$k \times 1.23 \times 1/3 \times (1-0.36)$ for the last third, plus $1.23 \times 1/3 \times 1.25$ for the Rank9 data structure.
In summary, xor+ filters use $1.0824 k + 0.5125 $~bits per entry as opposed to $1.23 k$~bit per entry for xor filters.


%\subsubsection{Storing User Data Instead of Fingerprints: Xor Map}

%The xor filter stores fingerprints for the approximate membership problem.
%As described in (Bloomier filter) and (Dietzfelbinger and Pagh), the same data structure can be used to store user-supplied data. This turns the xor filter into an immutable map, we call it the "xor map".

%Example use cases: For a collection of first names, store whether it's a boy or a girl name. For an LSM-tree, in addition to fingerprint data, store the level index. For an order-preserving minimal perfect hash table, store the key index. This way, the xor map can be used to build a Bloomier filter.

%Xor maps can be combined with the space optimization technique described in section~\ref{xor+}.



\subsection{Space Comparison}

We compare the space usage of some of the most important filters in Fig.~\ref{fig:spaceusagetheory_b}.
Bloom filters are more space efficient than cuckoo filters at a false-positive probability of 0.4\% or higher.

For very low false-positive probabilities ($5.6 \times 10^{-6}$), cuckoo filters at full capacity use less space than xor filters. However, we are not aware of any system that uses such a low false-positive probability: most systems seem to use between 8 and 20~bits per key~\cite{Sears:2012:BGP:2213836.2213862,dharmapurikar2003deep}. Thus we expect xor and xor+ filters to use less memory in practice.

\begin{figure}
\subfloat[Space vs. false-positive probability]{
    \includegraphics[width=0.48\textwidth]{spaceusage_b.tikz}}
\subfloat[False-positive probability vs. space]{
    \includegraphics[width=0.48\textwidth]{ffpvsspace_b.tikz}}
\caption{\label{fig:spaceusagetheory_b} Theoretical memory usage for Bloom filters (optimized for space), cuckoo filter (at max. capacity) and xor filters given a desired bound on the false-positive probability. }
\end{figure}


\section{Experiments}

We follow  Fan et al.'s testing procedure~\cite{Fan:2014:CFP:2674005.2674994}; we started from their software project~\cite{githubCuckoofilter}. 
% \hl{I think this needs to be said, that we started from their code.
% Thomas: I agree.}
Like them,  we use 64-bit keys as set elements. 
We build a filter based on a set of 10M or 100M keys.
We build a distinct set made of 10M queried keys. This set of queried keys is created by mixing some of
the keys from the original set, and some keys not present in the original set. We use different fractions (e.g., 0\%, 25\%, 50\%, 75\% and 100\%) of the keys  in the original set. The benchmark  counts the number of queried keys that are possibly in the set according to the filter. 
The benchmark is single threaded and calls the membership-test functions with different keys in a loop. We disable inlining of the functions to prevent compilers from 
unduly optimizing the benchmark which counts the number of matching keys. 

We run benchmarks on Intel processors with Skylake microarchitecture: 
an Intel i7-6700 processor running at 3.4\,GHz, with 8\,MB of L3 cache.
The software is compiled with the GNU~GCC~8.1.0 compiler to a 64-bit Linux executable with the flags \texttt{-O3 -march=native}.
For each filter, we run 3~tests, and report the median. 
Our error margin is less than 3\%.
The C++ source code of the filter implementations
and the benchmark is available\footnote{\url{https://github.com/FastFilter/fastfilter_cpp} (release 1.0), see ``Benchmarking'' section.}.
For some algorithms including all the xor and xor+ filters, we have also implemented Java versions\footnote{\url{https://github.com/FastFilter/fastfilter_java}} and well as a Go version\footnote{\url{https://github.com/FastFilter/xorfilter}}  and a pure C version\footnote{\url{https://github.com/FastFilter/xor_singleheader}},
but the benchmarks are using C++.

For all implementations, we use a randomly seeded Murmur finalizer~\cite{ivanchykhin2017regular} to compute the fingerprint from the key, as described in Algorithm~\ref{alg:hash}. We choose this option instead of faster alternatives so that even non-random keys work well and do not result in higher-than-expected false-positive probabilities, or construction failure  in the case of the cuckoo filter. For our tests, we use pseudo-randomly generated keys; we also tested with sequentially generated keys and found no statistically significant difference compared to using random keys after introducing the Murmur finalizer.

%\hl{Thomas: I added the following, I'm not sure if it's worth adding a separate algorithm for it.}
All implementations need to reduce a hash value $x$ to the range $\{0,\ldots,m - 1\}$ where $m$ is not necessarily a power of two.
Where this is needed,  we do not use the relatively slow modulo operation $x \mod m$ for performance reasons.
Instead, starting with  32-bit values $x$ and $m$ and computing their full 64-bit product $x \times m$, we use the faster multiply-shift combination $(x \times m) \div {2^{32}} = (x \times m) \mathrm{~>>~} 32$~\cite{Lemire:2019:FRI:3309768.3230636}.
%\hl{Thomas: I simplified this a bit by removing n}
%$index = ((hash~\&~((1 << 32) - 1)) * arrayLength) >> 32$ instead of modulo $index = hash~\%~arrayLength$. 

\begin{algorithm}
\caption{64-bit hash function\label{alg:hash}}
\begin{algorithmic}
    \REQUIRE key $x$, seed $s$
    \STATE $h \leftarrow x + s$
    \STATE $h \leftarrow (h \xor (h >> 33)) * \mathrm{0xff51afd7ed558ccd}$
    \STATE $h \leftarrow (h \xor (h >> 33)) * \mathrm{0xc4ceb9fe1a85ec53}$
    \STATE \textbf{return} $h \xor (h >> 33)$
\end{algorithmic}
\end{algorithm}


%\hl{Application: the "known passwords" database. TODO how to best present this? Convert it from Java to C++?}  
%\url{https://haveibeenpwned.com/passwords}.
%It covers 551,509,767 known password.
%Support for it is currently implemented in the Java version, \url{https://github.com/FastFilter/fastfilter_java#password-lookup-tool}.
%A segmented filter is used: the filter consists of $2^10$ xor+ filters, and the the highest 10 bits of the key decide which segment a key is stored.
%This slightly slows down lookup, but greatly reduces memory usage during construction, and speeds up construction if the keys are available in sorted order.

\subsection{Filter Implementations}

We run tests against the following filters:

\begin{itemize}

\item Bloom filter: We implemented the standard Bloom filter algorithm with configurable  false-positive probability (FPP) and size. We test with 8, 12, and 16 bits per key, and the respective number of hash functions $k$ that are needed for the lowest false-positive probability. For fast construction and membership test, we hash only once with a 64-bit function, treated as two 32-bit values $h_1(k)$ and $h_2(k)$. The Bloom filter hash functions are $g_i(k) = h_1(k) +i \cdot h_2(k)$ for $i=0,\ldots,k-1$. 
%\hl{We say that we implemented them, is that from Fan et al.'s, and if not, why did we go out and implement our own? 
%Thomas: they didn't include the Bloom filter implementation they used
%in their github project. Not sure why.
%My implementation is similar to the Google Guava one:
%https://github.com/google/guava/blob/master/guava/src/com/google/common/hash/BloomFilterStrategies.java#L113
%but I think I saw the same logic used in other implementations.
%I didn't find a good implementation so far.
%Now I saw there are multiple implementations in Apache Impala, but
%even those are not fully optimal (some use modulo).
%}
%\hl{Thomas: now i is 0..k-1, this may be a bit ugly...}
%The same as in all our other filter implementations, to calculate the array index, we use the faster multiply and shift combination
%$index = ((hash~\&~((1 << 32) - 1)) * arrayLength) >> 32$ instead of modulo $index = hash~\%~arrayLength$. 

% To speed up construction, we split the set into blocks of $2^{15}$ elements, where for each block we first calculate the bit indexes of the bits that need to be set, and then set all the respective bits, before processing the next block. 

%\hl{that's branchy Bloom or branchless? branchy, right?} 
%- \hl{Thomas: The implementation I listed in the benchmark results is the branchy one (one branch per bit). That's the "standard" one. The fastest "branch-less" one (uses two fewer branches than the  standard one) would be about 5\%-10\% faster, but the implementation is more complex. Listing that one would make the cuckoo filter look a tiny bit worse... Also, under "construction speed" I listed the one without the "addAll" optimization, so I removed that section.}

\item Blocked Bloom filter: We use a highly optimized blocked Bloom filter from Apache Impala\footnote{\url{https://impala.apache.org}}, which is also used in the cuckoo filter software project~\cite{githubCuckoofilter}. We modified it so the size is flexible and not restricted to $2^n$. It is designed for Intel AVX2 256-bit  operations; it is written using low-level Intel intrinsic functions. The advantage of this algorithm is the membership-test speed: each membership test is resolved from one cache line only using few instructions. The main disadvantage is that it is larger than regular Bloom filters.
%\hl{Wait? I thought that the implementation is from the Apache Impala project?}
%- \hl{Thomas: you are right! Now I wrote it's from Apache Impala, but kept that it's used in the cuckoo filter project, so that people know we didn't use an inferior implementation.}

% \item Original cuckoo filter (no shown in diagrams): We used the cuckoo filter implementation from the original authors~\cite{githubCuckoofilter}. We reduce the maximum load from 0.96 to 0.94, as otherwise construction can fail. The reduced maximum load is the recommended workaround suggested by the team that invented the cuckoo filter, but it is somewhat arbitrary; it resolved construction problems for our tests, but it is outside the scope of this paper to evaluate whether this  always work. The size of the filter is restricted to be a power of 2, which means that depending on the size of the set, up to 50\% of the space is unused, leading to a space overhead of up to 150\% in the worst case (for example, for a set of size 1980000). While it is faster than an implementation with a fixed space overhead, for a static set, wasting so much space seems problematic, specially as it doesn't improve the false-positive probability.

% \hl{If it is not reported, then omit it.}
% - \hl{Thomas: not sure what you refer to with "it"... is it "reduce the maximum load from 0.96 to 0.94"? This is reported in the cuckoo filter github project as an issue, and the recommendation is to reduce load.}
% - \hl{I will email you}

% \item Cuckoo filter (C) with flexible size: We used the cuckoo filter reference implementation from above,
% and modified so the size is flexible and not restricted to $2^n$. This required us to slightly change the calculation for the alternate location
% $l_2(x)$ for a key $x$ from the first location $l_1(x)$ and the fingerprint $f(x)$.
% Instead of $l_2(x) = l_1(x) \xor h(f(x))$,
% we use $l_2(x) = bucketCount - l_1(x) - h(f(x))$, and if the result is negative we add $bucketCount$.
% Due to the needed changes, the lookup performance (compared to the original cuckoo filter) is slightly reduced.

\item Cuckoo filter (C): We started with the cuckoo filter implementation from the original authors~\cite{githubCuckoofilter}. 
We reduce the maximum load from 0.96 to 0.94, as otherwise construction occasionally fails. The reduced maximum load is apparently the recommended workaround suggested by the cuckoo filter authors. Though it is outside our scope to evaluate whether it is always a reliable  fix, it was sufficient in our case. This reduction of the maximum load slightly worsens ($\approx $2\%) the memory usage of cuckoo filters. 
% \hl{added the above sentence to make it clear that it has bad consequences
% Thomas: I think it also improved construction speed, but I don't think that's important.}
In the original reference implementation~\cite{Fan:2014:CFP:2674005.2674994}, the size of the filter is restricted to be a power of two, which means up to 50\% of the space is unused. Wasting so much space seems problematic, especially since it does not improve the false-positive probability. Therefore, we modified it so the size is flexible and not restricted to $2^n$. This required us to slightly change the calculation for the alternate location $l_2(x)$ for a key $x$ from the first location $l_1(x)$ and the fingerprint $f(x)$. Instead of $l_2(x) = l_1(x) \xor h(f(x))$ as in Fan et al.~\cite{Fan:2014:CFP:2674005.2674994}, we use $l_2(x) = \mathrm{bucketCount} - l_1(x) - h(f(x))$, and if the result is negative we add $\mathrm{bucketCount}$.
We use 12-bit and 16-bit fingerprints.
%Due to the needed changes, the lookup performance (compared to the original cuckoo filter) is slightly reduced.

%\hl{Thomas: I combined the two "cuckoo filter" items now. Possibly we can shrink it a bit, but I think it's important that readers can follow the reasons behind the changes, and for that, maybe a bit of redundancy in the description is good... Not sure.}

\item Cuckoo semi-sorted (Css): We use the semi-sorted cuckoo filter reference implementation, modified in the same way as the regular cuckoo filter. From the original Fan et al.~\cite{Fan:2014:CFP:2674005.2674994} source release, we could only get one variant to work correctly, the version with a fingerprint size of 13~bits. Other versions have a non-zero false negative probability. 

\item Golomb-compressed sequence (GCS): Our implementation uses an average bucket size of 16, and Golomb Rice coding. We use a fingerprint size of 8~bits. %Unfortunately, we were not able to reach a competitive lookup performance. %, so we do not include the results in our graph.

\item Xor: Our xor and xor+ filters as described in \S~\ref{xor}. We use 8-bit and 16-bit fingerprints. 
%We tested with 8-bit and 16-bit fingerprints. 
%\hl{This is not consistent, sometimes Xor12 is included, sometimes it is not included. I suggest to omit it.}
%- \hl{Thomas: I removed it now.}

\end{itemize}

%\subsection{Experiment Setup}

\subsection{Construction Performance}

We present the construction times for 10~million and 100~million keys in Table~\ref{table:constructionTimeNsKey}. 
%We believe construction time is not critical for the static use case, especially if it is a background task. 
All construction algorithms are single-threaded; we did not investigate multi-threaded construction. 
%Where possible, we used bulk construction algorithms.
%\hl{Thomas: I commented "Where possible, we used bulk construction algorithms." as for the Bloom filter, we list times for the regular (not addAll) version. Also, someone might say it's possible to do bulk add for cuckoo filter as well, which is technically true, but would be very complex I think.}
For reference, we also present the time needed to sort the 64-bit keys using the C++ standard sorting algorithm (\texttt{std::sort}), on the same platform.

During construction, the blocked Bloom filter is clearly the fastest data structure. For the 100~million case, the semi-sorted variant of the cuckoo filter is the slowest. Construction of the xor filter with our implementation is roughly half as fast as the cuckoo filter and the Bloom filter, which have similar performance.

\begin{table}
\caption{Construction time in nanoseconds per key, rounded to 10 nanoseconds.}\label{table:constructionTimeNsKey}
\begin{tabular}{lrr}
\toprule
algorithm & 10 million keys & 100 million keys \\
  \midrule
% 2019-04-01 Skylake 
Blocked Bloom & 10 ns/key & 20 ns/key \\
Bloom 8 & 40 ns/key & 70 ns/key \\
Bloom 12 & 60 ns/key & 90 ns/key \\
Bloom 16 & 90 ns/key & 130 ns/key \\
Cuckoo semiSort 13 & 130 ns/key & 200 ns/key \\
Cuckoo 12 & 80 ns/key & 130 ns/key \\
Cuckoo 16 & 90 ns/key & 120 ns/key \\
GCS & 160 ns/key & 190 ns/key \\
Xor 8 & 110 ns/key & 130 ns/key \\
Xor 16 & 120 ns/key & 130 ns/key \\
Xor+ 8 & 160 ns/key & 180 ns/key \\
Xor+ 16 & 160 ns/key & 180 ns/key \\
(Sorting the keys) & 80 ns/key & 90 ns/key \\  
  \bottomrule
\end{tabular}
\end{table}




\subsection{Query Time Versus Space Overhead}

We present the performance numbers for the case where 25\% of the searched entries are in the set in Fig.~\ref{fig:qtvsspc25},
and  in the case where all searched entries are in the set in  Fig.~\ref{fig:qtvsspc100}. 
The results are presented in tabular form in Table~\ref{table:lookupBenchmarkResults}, where we include the Golomb-compressed sequence.

\begin{table}
\caption{Membership-test benchmark results, 25\% find. Timings are in nanosecond per query. \label{table:lookupBenchmarkResults}}
\subfloat[10M keys]{
\begin{tabular}{lrrr}
\toprule
Name & Time (ns) & Bits/key & FPP  \\
\midrule
Blocked Bloom & 16 & 10.7 & 0.939  \\
Bloom 8 & 31 & 8.0 & 2.161  \\
Bloom 12 & 40 & 12.0 & 0.313 \\
Bloom 16 & 48 & 16.0 & 0.046 \\
Cuckoo semiSort 13 & 57 & 12.8 & 0.092  \\
Cuckoo 12 & 31 & 12.8 & 0.183  \\
Cuckoo 16 & 32 & 17.0 & 0.012 \\
GCS & 137 & 10.0 & 0.389  \\
Xor 8 & 23 & 9.8 & 0.389  \\
Xor 16 & 27 & 19.7 & 0.002 \\
Xor+ 8 & 36 & 9.2 & 0.390  \\
Xor+ 16 & 43 & 17.8 & 0.002  \\
\bottomrule
\end{tabular}
}
\subfloat[100M keys]{
\begin{tabular}{lrrrr}
\toprule
 & Time (ns) & Bits/key & FPP \\
\midrule
 & 20 & 10.7 & 0.941 \\
 & 53 & 8.0 & 2.205  \\
& 58 & 12.0 & 0.339  \\
 & 68 & 16.0 & 0.053  \\
  & 94 & 12.8 & 0.092 \\
 & 38 & 12.8 & 0.184  \\
& 37 & 17.0 & 0.011  \\
 & 220 & 10.0 & 0.390  \\
 & 32 & 9.8 & 0.391  \\
 & 33 & 19.7 & 0.001  \\
 & 64 & 9.2 & 0.389  \\
 & 65 & 17.8 & 0.002 \\
\bottomrule
\end{tabular}
}

\end{table}




Unlike xor and cuckoo filters, the Bloom filter membership-test timings are sensitive to the fraction of keys present in the set. When an entry is not in the set, only a few bits need to be accessed, until the query function finds an unset bit and returns.
The Bloom filter is slower if an entry exists in the set, as it has to check all bits; this is especially the case for low false-positive probabilities. See Fig.~\ref{fig:qtvsspc100}. %, with large $k$. 

% The the cuckoo filter only uses less space for small false-positive rates
%, for example the cuckoo filter with 8-bit fingerprints uses more space 
% and is slower than the blocked Bloom filter. 

%The cuckoo filter only uses less space for false-positive rates well below 1\%. See Fig.~\ref{fig:fppvsspace}. T



\begin{figure}
\subfloat[10M keys]{
    \includegraphics[width=0.49\textwidth]{timevsspace10M-25-find.tikz}
  }
  \subfloat[100M keys]{
  \includegraphics[width=0.49\textwidth]{timevsspace100M-25-find.tikz}
  }
  \caption{Query time vs.\ space overhead, 25\% find}
  \label{fig:qtvsspc25}
\end{figure}

\begin{figure}
\subfloat[10M keys]{
    \includegraphics[width=0.49\textwidth]{timevsspace10M.tikz}}
    \subfloat[100M keys]{
    \includegraphics[width=0.49\textwidth]{timevsspace100M.tikz}
}
  \caption{Query time vs.\ space overhead, 100\% find}
  \label{fig:qtvsspc100}
\end{figure}


%\subsection{False Positive Probability Versus Bits per Key}

Ignoring query time,
Fig.~\ref{fig:fppvsspace} shows that Cuckoo~12 (C12) has memory usage that is close to Bloom filters. The cuckoo filter only uses much less space than Bloom filters for false-positive probabilities well below 1\% (Cuckoo~16 or C16).
In our experiments, the cuckoo filter,
and the slower semi-sorted cuckoo filter (Css), always use more space than the xor filter.
These experimental results match the theoretical results presented in Fig.~\ref{fig:spaceusagetheory_b}.
%The cuckoo filter uses less space than the Bloom filter for false-positive rates of around 0.3\% and lower.

%\hl{Thomas: I re-wrote that (see commented text), as we don't list the 8-bit cuckoo filter results. Also, comparing the cuckoo filter to the blocked Bloom filter doesn't seem to make sense here, as everything is slower than the blocked Bloom filter...}

The xor filter provides good query-time performance while using little space, even for moderate false-positive probabilities.


\begin{figure}
\subfloat[10M keys]{
\includegraphics[width=0.49\textwidth]{fppvsbitslog10.tikz}
}
  \subfloat[100M keys]{
    \includegraphics[width=0.49\textwidth]{fppvsbitslog100.tikz}
}
\caption{FPP vs.\ space usage in bits/key, log scale FPP\label{fig:fppvsspace}}
\end{figure}

\subsection{Discussion}

We attribute the  good membership-test performance of xor filters mainly to the following reasons.
Xor filters use exactly 3~memory accesses, independent of the false-positive probability. These memory accesses
can be executed in parallel by the memory subsystem. The number of instructions meanwhile is small and
there are no branches.

%\begin{itemize}
%    \item .
%    \item The memory accesses can run in parallel, as the memory location can be determined from the key only.
%    \item Lookup needs very few instructions, and no branches.
%\end{itemize}

For a false-positive probability of 1\%, the standard Bloom filter needs more memory accesses for a match, 
and even more so for lower false-positive probabilities. 
The Bloom filter uses between 41~and 105~instructions per key, depending on the number of set bits set and false-positive probability.
For a miss (if the key is not in the set), on average fewer memory accesses are needed, but there might be mispredicted  branches with accompanying penalties.
%This is likely the reason why the Bloom filter is slightly slower than the xor filter in our benchmarks.
% \hl{Removed last sentence as it is unclear.}

The cuckoo filter uses exactly 2~memory accesses, and 66 to 68 instructions per key (depending on fingerprint size).
The xor filter uses exactly 3~memory accesses, but only about 48~instructions per key.
Processors execute complex machine instructions using low-level instructions called $\mu$ops.
A processor like our Skylake can support
up to 10~outstanding memory requests per core, limited by an instruction  reorder buffer of 200~$\mu$ops. In the absence of mispredicted branches and long dependency chains,  the capacity of the instruction buffer becomes a limitation~\cite{beamer2015locality}.
It is likely the reason why the cuckoo filter and the xor filter have similar membership-test performance.  That is, while the cuckoo filter has fewer memory accesses, it generates more instructions which makes it harder for the processor to fetch as many memory requests as it could.
%\hl{We have instrumented tests, I think we should know how many more instructions are involved, no?}
%- \hl{Thomas: I added number of instructions for xor, cuckoo and Bloom filter.}

In our benchmarks, the blocked Bloom filter is the only algorithm that is clearly faster than the xor filter. This is most likely due to only having one memory access, and highly optimized code, using SIMD instructions specific to recent x64 processors. It needs fewer memory accesses and fewer instructions than its competitors.  %It is unclear how much of this speed advantage will hold up for non-Intel processors, such as ARM and RISC-V.
It might be difficult to implement a similarly efficient approach in a higher-level language like Java, or using solely portable code. If memory usage or low false-positive probability are a primary concern, the blocked Bloom filter may not be a good choice.


While an xor filter is immutable, we believe that it is not a  limitation for many important applications; competitive alternatives all have limited mutability in any case. Approximate filters that support fast mergers or additions (e.g., Bloom filters) require the original filters to have extra capacity. The update may even fail in the case of Cuckoo filters. Re-building the filter can maintain an optimal size. In multithreaded systems, immutability avoids the overhead of synchronization mechanisms to maintain concurrency.

%\subsection{Space Usage}

%In all cases, the xor filter uses less space than competing algorithms. It even needs slightly less space than the semi-sorted cuckoo filter. The space saving  does not come with added complexity, or slower performance.

% Some thoughts shared by email:) Right. So from my analysis, if you make sure you do not have crazy prefetching, then you get that for out-of-cache, xor filters have 3 cache misses per key, against 2 cache misses per key for cuckoo filters. Yet xor filters still win out in the end because they have far fewer instructions per key (about half as many). It may seem like having  more cache misses is a terrible thing, but one must factor in memory-level parallelism. Recent Intel processors can sustain up to 10 concurrent cache transfers... so the 3 cache misses, when they occur nearly at the same time can translate into 3 concurrent cache transfers. So the number of cache misses is not necessarily the main determinant of performance.

% The way you have implemented Bloom filters, there are quite a few branch misses. You could reduce this number, but probably at the expense of more cache misses, so it is a difficult balancing act. The current implementation is probably standard and fine.

% (Is using more space is not a concern, then BlockedBloom is appealing.)

\section{Conclusion and Future Work}

Xor filters are typically faster than Bloom filters,
and they save about 15\% in memory usage. While the construction of xor filters is  slower than Bloom filters ($\approx 2 \times $), we expect that the construction is a one-time cost amortized over many queries. %the filters might be rarely updated in several applications. %While xor filter is immutable, we believe that it is not a serious limitation for many important applications; competitive alternatives all have limited mutability in any case.
Future work could consider batched queries~\cite{Breslow:2018:MFF:3213880.3232248} to improve performance. It might also be possible to partially parallelize the construction of the filters.

%\hl{It seems obvious to me that the first part of the mapping algorithm (the part that is actually quite expensive) can be parallelized over three cores quite naturally. That is, because $C$ and $H$ are effectively partitioned in separate memory regions, and $S$ is immutable, there is no reason why you cannot do it in parallel. But the computation of the fingerprints would then be three times, which is bad. So you would need, maybe, to introduce a step where you compute just the fingerprints, unless you can find that the computation of the fingerprints is sufficiently cheap (it might be).
%But then you can cut the problem another way: you can divide up $S$ into small chunks. So pick $N$~values from $S$, compute their fingerprints, then, in parallel do the counter and the XORing. Adjust the value $N$~accordingly (it should fit in L3 cache, evidently). The purpose of parallelization here would not be so much to save on computations per se, the computations are cheap, but rather to maximize memory bandwith.}

%\hl{My impression is that you might be able to speed the construction up by computing $h_1$, $h_2$ and $h_2$ once instead of twice in the mapping step. It is not so much the computation itself that is a problem, but by mixing computations within a stream of memory accesses, you reduce the ability of the processor to pipeline as many loads and stores as possible. Whether this makes a difference depends on the cost of computing  $h_1$, $h_2$ and $h_2$, evidently.}

%\hl{Thomas: I think single-threaded construction speed can be further improved by using a "blocked" / "batch" approach that is used currently for the first step (method applyBlock).}


\appendix
\section{Original Versus Compact Cuckoo Filters}
In Table~\ref{table:constructionTimeNsKeyTradeOff}, we compare the 
original implementations of cuckoo filters which require that the filter
size be a power of two, with our more compact implementation. Given 10~million keys, the memory usage of cuckoo filters using the original implementation is not competitive. However, the construction time 
is reduced with an overallocated filter because hash collisions are less frequent. Similarly, the query times (25\% of the entries in the set) are about 10\% smaller in the original implementation. However, if we choose a number of keys near a power of two (e.g., 31.5~million keys), the original and compact implementations have nearly the same memory usage, construction times, and query speeds.

\begin{table}
\caption{Construction time, memory usage and query time (25\% of the entries in the set) for original and compact cuckoo filters with 10 million keys.}\label{table:constructionTimeNsKeyTradeOff}
\begin{tabular}{rrrr}
\toprule
Name & Construction Time & Memory & Query Time \\
  \midrule
% 2019-04-01 Skylake 
Cuckoo 12 & 80 ns/key & 12.8~bits/key  & 31~ns/key\\
Cuckoo 12 (original) & 40 ns/key & 20.1~bits/key & 30~ns/key\\[0.2cm]
Cuckoo 16 & 90 ns/key & 17.0~bits/key  & 32~ns/key\\
Cuckoo 16 (original) & 40 ns/key & 26.8~bits/key & 28~ns/key\\
  \bottomrule
\end{tabular}
\end{table}


\section{Quotient  and Morton   Filters}
We consider quotient filters~\cite{Pandey:2017:GCF:3035918.3035963} (CQF) experimentally.
 We use the reference implementation~\cite{githubCQF}. The implementation
 relies on assembly code optimized for recent x64 processors.
 As with cuckoo filters, the original implementation requires that the capacity 
 be  a power of two. 
Table~\ref{table:cqflookupBenchmarkResults} shows that the query time of the reference quotient-filter implementation is several times the query time of competitive approaches like cuckoo or xor filters. We also consider Morton filters~\cite{Breslow:2018:MFF:3213880.3232248} with the reference implementation~\cite{githubMortonfilter}. Morton filters answer one-at-a-time  queries at half the speed of 8-bit xor filters, despite similar false-positive probabilities and memory usage. 

\begin{table}\centering
\caption{Performance of counting quotient filters (CQF) and Morton filters. We include Xor~8 results for comparison. For queries, we report the results corresponding to 25\% of the entries being in the set. \label{table:cqflookupBenchmarkResults} }
\begin{tabular}{lrrrr}
\toprule
Name & Query Time (ns/key) & Bits/key & FPP & volume \\
\midrule
Xor~8 & 23 & 9.8 & 0.39 & 10M \\
CQF & 64 & 17.0 & 0.23 & 10M \\
Morton & 47 & 11.7 & 0.31 & 10M \\\midrule
Xor~8 & 32 & 9.8 & 0.39 & 100M \\
CQF & 88 & 13.6 & 0.29 & 100M \\
Morton & 65 & 11.7 & 0.31 & 100M \\
\bottomrule
\end{tabular}
\end{table}


\appendix
\section{Performance on Different Processors}

We list the benchmark results for different processors.
The blocked Bloom filter and CQF implementations use Intel assembler instructions;
we did not port those to ARM, and so could not run those tests.
In all cases, 3 tests were run, and the medians are listed.

\hl{TODO do we need to list hardware specifications?}

\begin{table}[ht!]
\small
\begin{tabular}{lrrrrrrrrrr}
\hline
Name & Constr. & \multicolumn{5}{l}{Lookup} & Bits & FPP & Over- & Million \\
 & ns/key & 0\% &  25\% & 50\% & 75\% & 100\% & /key & & head & keys \\
\hline
% 2019-04-01
BlockedBloom & 13 & 16 & 16 & 16 & 16 & 16 & 13.4 & 0.317 & 61.7 & 10 \\
BlockedBloom-addAll & 16 & 16 & 16 & 16 & 16 & 16 & 10.7 & 0.939 & 58.4 & 10 \\
Bloom8 & 37 & 31 & 31 & 32 & 32 & 33 & 8.0 & 2.161 & 44.6 & 10 \\
Bloom12 & 62 & 37 & 40 & 43 & 47 & 50 & 12.0 & 0.313 & 44.3 & 10 \\
Bloom16 & 90 & 41 & 48 & 55 & 62 & 69 & 16.0 & 0.046 & 44.2 & 10 \\
Bloom8-addAll & 30 & 30 & 31 & 32 & 32 & 33 & 8.0 & 2.159 & 44.6 & 10 \\
Bloom12-addAll & 39 & 37 & 40 & 43 & 46 & 50 & 12.0 & 0.314 & 44.3 & 10 \\
Bloom16-addAll & 51 & 42 & 49 & 56 & 63 & 70 & 16.0 & 0.046 & 44.1 & 10 \\
BranchlessBloom8-addAll & 30 & 26 & 28 & 29 & 31 & 32 & 8.0 & 2.154 & 44.5 & 10 \\
BranchlessBloom12-addAll & 39 & 32 & 36 & 40 & 44 & 47 & 12.0 & 0.315 & 44.4 & 10 \\
BranchlessBloom16-addAll & 51 & 36 & 44 & 52 & 60 & 68 & 16.0 & 0.046 & 44.3 & 10 \\
CountingBloom10-addAll & 44 & 50 & 53 & 56 & 58 & 61 & 40.0 & 0.818 & 476.9 & 10 \\
CuckooSemiSort13 & 140 & 57 & 57 & 57 & 57 & 57 & 12.8 & 0.092 & 26.5 & 10 \\
Cuckoo8 & 66 & 25 & 25 & 25 & 25 & 25 & 8.5 & 2.915 & 66.9 & 10 \\
Cuckoo12 & 88 & 31 & 31 & 31 & 31 & 31 & 12.8 & 0.183 & 40.4 & 10 \\
Cuckoo16 & 94 & 32 & 32 & 32 & 32 & 32 & 17.0 & 0.012 & 30.0 & 10 \\
GCS & 165 & 137 & 137 & 138 & 138 & 138 & 10.0 & 0.389 & 25.4 & 10 \\
SimpleBlockedBloom & 35 & 35 & 35 & 35 & 36 & 36 & 10.9 & 0.961 & 62.6 & 10 \\
SuccCountBlockBloom10 & 124 & 23 & 25 & 26 & 28 & 30 & 23.6 & 1.004 & 255.5 & 10 \\
SuccCountingBloom10-addAll & 99 & 34 & 36 & 37 & 39 & 41 & 21.2 & 0.822 & 206.1 & 10 \\
Xor8 & 112 & 23 & 23 & 23 & 23 & 23 & 9.8 & 0.389 & 22.9 & 10 \\
Xor12 & 117 & 34 & 34 & 34 & 34 & 34 & 14.8 & 0.025 & 23.5 & 10 \\
Xor16 & 117 & 27 & 27 & 27 & 27 & 27 & 19.7 & 0.002 & 22.7 & 10 \\
Xor+8 & 156 & 36 & 36 & 36 & 36 & 36 & 9.2 & 0.390 & 14.4 & 10 \\
Xor+16 & 160 & 42 & 43 & 43 & 43 & 43 & 17.8 & 0.002 & 12.7 & 10 \\
BlockedBloom & 18 & 19 & 19 & 19 & 19 & 19 & 10.7 & 0.913 & 58.5 & 100 \\
BlockedBloom-addAll & 17 & 20 & 20 & 20 & 20 & 20 & 10.7 & 0.941 & 58.5 & 100 \\
Bloom8 & 68 & 53 & 53 & 53 & 53 & 53 & 8.0 & 2.205 & 45.4 & 100 \\
Bloom12 & 94 & 53 & 58 & 63 & 68 & 73 & 12.0 & 0.339 & 46.2 & 100 \\
Bloom16 & 130 & 56 & 68 & 80 & 92 & 104 & 16.0 & 0.053 & 47.1 & 100 \\
Bloom8-addAll & 32 & 53 & 53 & 53 & 54 & 54 & 8.0 & 2.197 & 45.2 & 100 \\
Bloom12-addAll & 46 & 53 & 58 & 63 & 68 & 74 & 12.0 & 0.338 & 46.2 & 100 \\
Bloom16-addAll & 69 & 56 & 68 & 80 & 92 & 105 & 16.0 & 0.053 & 47.2 & 100 \\
BranchlessBloom8-addAll & 32 & 46 & 47 & 49 & 51 & 53 & 8.0 & 2.199 & 45.3 & 100 \\
BranchlessBloom12-addAll & 46 & 46 & 53 & 59 & 66 & 73 & 12.0 & 0.338 & 46.2 & 100 \\
BranchlessBloom16-addAll & 69 & 48 & 63 & 76 & 90 & 104 & 16.0 & 0.054 & 47.3 & 100 \\
CountingBloom10-addAll & 102 & 59 & 63 & 67 & 71 & 75 & 40.0 & 0.848 & 481.2 & 100 \\
CuckooSemiSort13 & 204 & 94 & 94 & 94 & 94 & 94 & 12.8 & 0.092 & 26.5 & 100 \\
Cuckoo8 & 126 & 37 & 37 & 37 & 37 & 37 & 8.5 & 2.916 & 66.9 & 100 \\
Cuckoo12 & 130 & 38 & 38 & 38 & 38 & 38 & 12.8 & 0.184 & 40.5 & 100 \\
Cuckoo16 & 128 & 37 & 37 & 37 & 37 & 37 & 17.0 & 0.011 & 29.8 & 100 \\
GCS & 186 & 220 & 220 & 220 & 220 & 220 & 10.0 & 0.390 & 25.5 & 100 \\
SimpleBlockedBloom & 52 & 52 & 53 & 53 & 53 & 52 & 10.9 & 0.964 & 62.7 & 100 \\
SuccCountBlockBloom10 & 147 & 32 & 36 & 40 & 44 & 48 & 23.6 & 1.004 & 255.5 & 100 \\
SuccCountingBloom10-addAll & 112 & 53 & 55 & 58 & 60 & 63 & 21.2 & 0.849 & 208.2 & 100 \\
Xor8 & 127 & 32 & 32 & 32 & 32 & 32 & 9.8 & 0.391 & 23.0 & 100 \\
Xor12 & 130 & 43 & 43 & 43 & 43 & 43 & 14.8 & 0.025 & 23.1 & 100 \\
Xor16 & 129 & 33 & 33 & 33 & 33 & 33 & 19.7 & 0.001 & 22.4 & 100 \\
Xor+8 & 181 & 64 & 64 & 64 & 64 & 64 & 9.2 & 0.389 & 14.4 & 100 \\
Xor+16 & 183 & 65 & 65 & 65 & 65 & 65 & 17.8 & 0.002 & 12.1 & 100 \\
\hline
\end{tabular}
\caption{Experimental results, Intel Skylake processor \hl{TODO cleanup list; show hardware specs}}
\label{tab:resultsSkylake}
\end{table}

\begin{table}
\small
\begin{tabular}{lrrrrrrrrrr}
\hline
Name & Constr. & \multicolumn{5}{l}{Lookup} & Bits & FPP & Over- & Million \\
 & ns/key & 0\% &  25\% & 50\% & 75\% & 100\% & /key & & head & keys \\
\hline
BlockedBloom & 21 & 19 & 19 & 19 & 19 & 19 & 10.7 & 0.944 & 58.5 & 10 \\
Bloom8 & 47 & 34 & 35 & 36 & 37 & 38 & 8.0 & 2.158 & 44.5 & 10 \\
Bloom12 & 77 & 42 & 46 & 50 & 55 & 59 & 12.0 & 0.314 & 44.3 & 10 \\
Bloom16 & 111 & 47 & 58 & 68 & 78 & 88 & 16.0 & 0.046 & 44.5 & 10 \\
CQF & 151 & 75 & 88 & 101 & 114 & 127 & 17.0 & 0.234 & 94.8 & 10 \\
CuckooSemiSort13 & 176 & 74 & 74 & 74 & 74 & 74 & 12.8 & 0.091 & 26.3 & 10 \\
Cuckoo8 & 83 & 31 & 31 & 31 & 31 & 31 & 8.5 & 2.909 & 66.8 & 10 \\
Cuckoo12 & 107 & 40 & 40 & 40 & 40 & 40 & 12.8 & 0.182 & 40.2 & 10 \\
Cuckoo16 & 113 & 41 & 41 & 41 & 41 & 41 & 17.0 & 0.012 & 30.1 & 10 \\
GCS & 186 & 165 & 165 & 165 & 165 & 165 & 10.0 & 0.391 & 25.5 & 10 \\
Xor8 & 204 & 28 & 28 & 28 & 28 & 28 & 9.8 & 0.389 & 22.9 & 10 \\
Xor12 & 208 & 42 & 42 & 42 & 42 & 42 & 14.8 & 0.025 & 23.2 & 10 \\
Xor16 & 207 & 33 & 33 & 33 & 33 & 33 & 19.7 & 0.002 & 22.5 & 10 \\
Xor+8 & 204 & 40 & 40 & 40 & 40 & 41 & 9.2 & 0.435 & 16.6 & 10 \\
Xor+16 & 213 & 48 & 48 & 48 & 48 & 48 & 17.8 & 0.002 & 15.4 & 10 \\
BlockedBloom & 28 & 25 & 24 & 25 & 24 & 25 & 10.7 & 0.945 & 58.6 & 100 \\
Bloom8 & 84 & 59 & 61 & 63 & 65 & 67 & 8.0 & 2.208 & 45.4 & 100 \\
Bloom12 & 114 & 59 & 66 & 74 & 81 & 89 & 12.0 & 0.337 & 46.1 & 100 \\
Bloom16 & 158 & 62 & 78 & 93 & 110 & 125 & 16.0 & 0.053 & 47.0 & 100 \\
CQF & 196 & 110 & 125 & 141 & 157 & 173 & 13.6 & 0.291 & 61.4 & 100 \\
CuckooSemiSort13 & 254 & 118 & 118 & 118 & 118 & 118 & 12.8 & 0.092 & 26.6 & 100 \\
Cuckoo8 & 155 & 46 & 46 & 46 & 46 & 46 & 8.5 & 2.909 & 66.8 & 100 \\
Cuckoo12 & 156 & 48 & 48 & 48 & 48 & 49 & 12.8 & 0.184 & 40.5 & 100 \\
Cuckoo16 & 157 & 48 & 48 & 48 & 48 & 48 & 17.0 & 0.012 & 30.2 & 100 \\
GCS & 212 & 272 & 273 & 273 & 271 & 271 & 10.0 & 0.390 & 25.5 & 100 \\
Xor8 & 231 & 38 & 38 & 38 & 38 & 38 & 9.8 & 0.389 & 22.9 & 100 \\
Xor12 & 236 & 51 & 51 & 51 & 51 & 51 & 14.8 & 0.024 & 22.9 & 100 \\
Xor16 & 234 & 41 & 41 & 41 & 41 & 41 & 19.7 & 0.002 & 23.3 & 100 \\
Xor+8 & 234 & 69 & 69 & 70 & 70 & 70 & 9.2 & 0.395 & 14.7 & 100 \\
Xor+16 & 235 & 72 & 72 & 73 & 73 & 74 & 17.8 & 0.003 & 18.9 & 100 \\
\hline
\end{tabular}
\caption{Experimental results, Intel Skylake X processor \hl{TODO re-run tests; cleanup list; show hardware specs}}
\label{tab:resultsSkylakeX}
\end{table}

\begin{table}
\small
\begin{tabular}{lrrrrrrrrrr}
\hline
Name & Constr. & \multicolumn{5}{l}{Lookup} & Bits & FPP & Over- & Million \\
 & ns/key & 0\% &  25\% & 50\% & 75\% & 100\% & /key & & head & keys \\
\hline
% 2019-04-01 Ampere
BlockedBloom & 54 & 69 & 69 & 69 & 69 & 69 & 12.8 & 0.636 & 75.4 & 10 \\
Bloom8 & 67 & 65 & 66 & 67 & 68 & 69 & 8.0 & 2.155 & 44.5 & 10 \\
Bloom12 & 87 & 67 & 71 & 73 & 77 & 80 & 12.0 & 0.316 & 44.4 & 10 \\
Bloom16 & 141 & 69 & 85 & 100 & 115 & 130 & 16.0 & 0.047 & 44.5 & 10 \\
Bloom8-addAll & 71 & 67 & 68 & 69 & 70 & 71 & 8.0 & 2.155 & 44.5 & 10 \\
Bloom12-addAll & 95 & 67 & 71 & 74 & 77 & 80 & 12.0 & 0.316 & 44.4 & 10 \\
Bloom16-addAll & 128 & 70 & 85 & 98 & 114 & 127 & 16.0 & 0.046 & 44.4 & 10 \\
BranchlessBloom8-addAll & 69 & 50 & 57 & 65 & 73 & 81 & 8.0 & 2.157 & 44.5 & 10 \\
BranchlessBloom12-addAll & 93 & 50 & 64 & 79 & 93 & 109 & 12.0 & 0.314 & 44.3 & 10 \\
BranchlessBloom16-addAll & 130 & 56 & 82 & 109 & 136 & 163 & 16.0 & 0.046 & 44.3 & 10 \\
CountingBloom10-addAll & 108 & 97 & 116 & 135 & 153 & 172 & 40.0 & 0.815 & 476.5 & 10 \\
CuckooSemiSort13 & 208 & 80 & 80 & 80 & 80 & 80 & 12.8 & 0.092 & 26.6 & 10 \\
Cuckoo8 & 155 & 67 & 67 & 67 & 67 & 67 & 8.5 & 2.918 & 66.9 & 10 \\
Cuckoo12 & 168 & 70 & 70 & 71 & 70 & 70 & 12.8 & 0.182 & 40.2 & 10 \\
Cuckoo16 & 162 & 73 & 72 & 72 & 72 & 73 & 17.0 & 0.011 & 29.7 & 10 \\
GCS & 216 & 240 & 240 & 240 & 240 & 239 & 10.0 & 0.391 & 25.5 & 10 \\
SimpleBlockedBloom & 75 & 70 & 70 & 70 & 70 & 70 & 10.9 & 0.958 & 62.5 & 10 \\
SuccCountBlockBloom10 & 486 & 42 & 49 & 56 & 63 & 70 & 23.6 & 1.006 & 255.7 & 10 \\
SuccCountingBloom10-addAll & 569 & 69 & 76 & 83 & 90 & 97 & 21.2 & 0.818 & 205.8 & 10 \\
Xor8 & 319 & 46 & 47 & 47 & 47 & 47 & 9.8 & 0.392 & 23.1 & 10 \\
Xor12 & 330 & 65 & 65 & 65 & 65 & 65 & 14.8 & 0.024 & 22.8 & 10 \\
Xor16 & 324 & 52 & 52 & 51 & 52 & 52 & 19.7 & 0.001 & 22.3 & 10 \\
Xor+8 & 313 & 122 & 122 & 122 & 122 & 122 & 9.2 & 0.391 & 14.4 & 10 \\
Xor+16 & 347 & 131 & 132 & 132 & 132 & 132 & 17.8 & 0.001 & 10.8 & 10 \\
BlockedBloom & 97 & 121 & 121 & 121 & 121 & 121 & 12.8 & 0.635 & 75.4 & 100 \\
Bloom8 & 159 & 115 & 125 & 135 & 144 & 153 & 8.0 & 2.204 & 45.4 & 100 \\
Bloom12 & 222 & 125 & 145 & 165 & 185 & 204 & 12.0 & 0.338 & 46.2 & 100 \\
Bloom16 & 300 & 129 & 166 & 202 & 239 & 275 & 16.0 & 0.054 & 47.4 & 100 \\
Bloom8-addAll & 84 & 115 & 125 & 134 & 144 & 153 & 8.0 & 2.205 & 45.4 & 100 \\
Bloom12-addAll & 113 & 122 & 142 & 162 & 181 & 201 & 12.0 & 0.340 & 46.3 & 100 \\
Bloom16-addAll & 151 & 132 & 170 & 207 & 244 & 280 & 16.0 & 0.053 & 47.2 & 100 \\
BranchlessBloom8-addAll & 87 & 104 & 121 & 138 & 155 & 172 & 8.0 & 2.199 & 45.3 & 100 \\
BranchlessBloom12-addAll & 115 & 110 & 142 & 175 & 207 & 239 & 12.0 & 0.338 & 46.2 & 100 \\
BranchlessBloom16-addAll & 148 & 117 & 171 & 226 & 280 & 335 & 16.0 & 0.054 & 47.4 & 100 \\
CountingBloom10-addAll & 167 & 124 & 149 & 175 & 201 & 227 & 40.0 & 0.851 & 481.6 & 100 \\
CuckooSemiSort13 & 310 & 153 & 153 & 153 & 153 & 157 & 12.8 & 0.092 & 26.5 & 100 \\
Cuckoo8 & 242 & 127 & 127 & 127 & 127 & 127 & 8.5 & 2.916 & 66.9 & 100 \\
Cuckoo12 & 254 & 132 & 132 & 132 & 132 & 136 & 12.8 & 0.182 & 40.3 & 100 \\
Cuckoo16 & 263 & 142 & 142 & 142 & 142 & 142 & 17.0 & 0.011 & 29.8 & 100 \\
GCS & 240 & 312 & 313 & 313 & 312 & 314 & 10.0 & 0.389 & 25.5 & 100 \\
SimpleBlockedBloom & 124 & 118 & 118 & 118 & 118 & 118 & 10.9 & 0.961 & 62.5 & 100 \\
SuccCountBlockBloom10 & 592 & 68 & 79 & 91 & 102 & 114 & 23.6 & 1.010 & 256.0 & 100 \\
SuccCountingBloom10-addAll & 603 & 120 & 141 & 162 & 183 & 203 & 21.2 & 0.848 & 208.1 & 100 \\
Xor8 & 329 & 105 & 105 & 105 & 105 & 105 & 9.8 & 0.390 & 22.9 & 100 \\
Xor12 & 345 & 151 & 151 & 151 & 151 & 151 & 14.8 & 0.024 & 22.8 & 100 \\
Xor16 & 339 & 108 & 108 & 108 & 108 & 107 & 19.7 & 0.001 & 22.2 & 100 \\
Xor+8 & 332 & 204 & 204 & 204 & 204 & 205 & 9.2 & 0.392 & 14.5 & 100 \\
Xor+16 & 350 & 221 & 221 & 221 & 220 & 220 & 17.8 & 0.001 & 10.6 & 100 \\
\hline
\end{tabular}
\caption{Experimental results, 64-bit ARM \hl{Ampere TODO cleanup list; show hardware specs}.}
\label{tab:resultsARM}
\end{table}

\end{document}










===============


% new results ---------------------------------------
\hl{Thomas: Lookup for original cuckoo are a tiny bit faster, but it doesn't change the picture much.
Morton lookup is slower than cuckoo, as was expected (the authors say that batched lookup is faster, and we don't do batched lookup).
For some reason (I didn't investigate), Original CuckooSemiSort13 is slower than modified CuckooSemiSort13, at 10 million keys.
}
\begin{table}[]
\small
\begin{tabular}{lrrrrrrrrrr}
\hline
Name & Constr. & \multicolumn{5}{l}{Lookup} & bits & False & over- & Million \\
 & ns/key & 0\% &  25\% & 50\% & 75\% & 100\% & /key & positives & head & keys \\
\hline
BlockedBloom & 12 & 16 & 16 & 16 & 16 & 16 & 10.7 & 0.941 & 58.4 & 10 \\
Bloom8 & 36 & 29 & 29 & 30 & 31 & 32 & 8.0 & 2.152 & 44.4 & 10 \\
Bloom12 & 60 & 36 & 39 & 43 & 46 & 50 & 12.0 & 0.314 & 44.3 & 10 \\
Bloom16 & 88 & 39 & 46 & 53 & 60 & 68 & 16.0 & 0.047 & 44.9 & 10 \\
CQF & 106 & 55 & 64 & 73 & 81 & 90 & 17.0 & 0.232 & 94.5 & 10 \\
CuckooSemiSort13 & 133 & 55 & 55 & 55 & 55 & 55 & 12.8 & 0.092 & 26.6 & 10 \\
Cuckoo12 & 84 & 30 & 30 & 30 & 30 & 30 & 12.8 & 0.183 & 40.3 & 10 \\
Cuckoo16 & 89 & 31 & 31 & 31 & 31 & 31 & 17.0 & 0.012 & 30.0 & 10 \\
GCS & 153 & 134 & 131 & 131 & 131 & 131 & 10.0 & 0.390 & 25.5 & 10 \\
Morton & 51 & 46 & 47 & 48 & 49 & 50 & 11.7 & 0.311 & 40.7 & 10 \\
Original Cuckoo12 & 41 & 30 & 30 & 30 & 30 & 30 & 20.1 & 0.117 & 106.7 & 10 \\
Original Cuckoo16 & 39 & 28 & 28 & 28 & 28 & 28 & 26.8 & 0.007 & 95.5 & 10 \\
Original CuckooSemiSort13 & 89 & 65 & 65 & 65 & 65 & 65 & 20.1 & 0.058 & 87.3 & 10 \\
Xor8 & 106 & 23 & 23 & 23 & 23 & 23 & 9.8 & 0.390 & 23.0 & 10 \\
Xor16 & 112 & 27 & 27 & 27 & 27 & 27 & 19.7 & 0.002 & 22.9 & 10 \\
Xor+8 & 148 & 34 & 34 & 34 & 34 & 34 & 9.2 & 0.392 & 14.5 & 10 \\
Xor+16 & 153 & 41 & 41 & 41 & 41 & 41 & 17.8 & 0.002 & 11.7 & 10 \\
BlockedBloom & 18 & 21 & 21 & 21 & 21 & 21 & 10.7 & 0.942 & 58.5 & 100 \\
Bloom8 & 66 & 50 & 50 & 50 & 51 & 51 & 8.0 & 2.204 & 45.3 & 100 \\
Bloom12 & 90 & 52 & 57 & 62 & 66 & 71 & 12.0 & 0.339 & 46.2 & 100 \\
Bloom16 & 126 & 53 & 64 & 76 & 87 & 98 & 16.0 & 0.054 & 47.5 & 100 \\
CQF & 140 & 78 & 88 & 98 & 109 & 119 & 13.6 & 0.292 & 61.5 & 100 \\
CuckooSemiSort13 & 196 & 91 & 91 & 91 & 91 & 91 & 12.8 & 0.091 & 26.3 & 100 \\
Cuckoo12 & 125 & 37 & 37 & 37 & 37 & 37 & 12.8 & 0.184 & 40.4 & 100 \\
Cuckoo16 & 123 & 36 & 36 & 36 & 36 & 36 & 17.0 & 0.012 & 30.5 & 100 \\
GCS & 171 & 213 & 213 & 213 & 213 & 213 & 10.1 & 0.390 & 25.6 & 100 \\
Morton & 60 & 64 & 65 & 66 & 68 & 69 & 11.7 & 0.312 & 40.8 & 100 \\
Original Cuckoo12 & 58 & 34 & 34 & 34 & 34 & 34 & 16.1 & 0.146 & 71.0 & 100 \\
Original Cuckoo16 & 56 & 32 & 32 & 32 & 32 & 32 & 21.5 & 0.009 & 59.9 & 100 \\
Original CuckooSemiSort13 & 125 & 92 & 92 & 92 & 92 & 92 & 16.1 & 0.073 & 54.4 & 100 \\
Xor8 & 121 & 31 & 31 & 31 & 31 & 31 & 9.8 & 0.388 & 22.9 & 100 \\
Xor16 & 123 & 32 & 32 & 32 & 32 & 32 & 19.7 & 0.002 & 23.2 & 100 \\
Xor+8 & 171 & 61 & 61 & 61 & 61 & 61 & 9.2 & 0.390 & 14.4 & 100 \\
Xor+16 & 174 & 62 & 62 & 63 & 63 & 63 & 17.8 & 0.002 & 12.1 & 100 \\
\hline
\end{tabular}
\end{table}
% new results ---------------------------------------


% new results ---------------------------------------
\hl{Thomas: 
Construction for original cuckoo filters are much faster at 10 and 100 million keys
because the load factor is very slow in both cases. 
At 31.5 million keys, where load factor is similar, 
the construction times are very similar; 
original cuckoo is 5\% faster. 

For Morton filter, the batch-add method is used.
}

\begin{table}
\caption{Construction time in nanoseconds per key, rounded to 10 nanoseconds.}\label{table:constructionTimeNsKey2}
\begin{tabular}{lrr}
\toprule
algorithm & 10 million keys & 100 million keys \\
  \midrule
% 2019-08-24 Skylake
BlockedBloom & 10 ns/key & 20 ns/key \\
Bloom 8 & 40 ns/key & 70 ns/key \\
Bloom 12 & 60 ns/key & 90 ns/key \\
Bloom 16 & 90 ns/key & 130 ns/key \\
Counting quotient filter & 110 ns/key & 140 ns/key \\
Cuckoo semiSort 13 & 130 ns/key & 200 ns/key \\
Cuckoo 12 & 80 ns/key & 130 ns/key \\
Cuckoo 16 & 90 ns/key & 120 ns/key \\
Golomb compressed set & 150 ns/key & 170 ns/key \\
Morton 3/8 & 50 ns/key & 60 ns/key \\
Original Cuckoo 12 & 40 ns/key & 60 ns/key \\
Original Cuckoo 16 & 40 ns/key & 60 ns/key \\
Original Cuckoo semiSort 13 & 90 ns/key & 120 ns/key \\
Xor 8 & 110 ns/key & 120 ns/key \\
Xor 16 & 110 ns/key & 120 ns/key \\
Xor+ 8 & 150 ns/key & 170 ns/key \\
Xor+ 16 & 150 ns/key & 170 ns/key \\
(Sorting the keys) & 80 ns/key & 90 ns/key \\
  \bottomrule
\end{tabular}
\end{table}
% new results ---------------------------------------

It seems extraordinary that the 4-wise binary fuse is faster than Xor. We are going to have to explain that.
Zen 2
$ ./bulk-insert-and-query.exe 10000000 0,98,100                                                    find    find    find    find    find  1*add+                       optimal  wasted million                                     add  remove      0%     25%     50%     75%    100%  3*find      ε%  bits/item  bits/item  space%    keys
                            Xor8  123.38    0.00    9.17    9.19    9.14    9.21    9.32  151.00  0.3900       9.84       8.00    23.0  10.000XorBinaryFuseFilter8-4WisePrefetch   91.40    0.00    7.63    7.63    7.63    7.61    7.71  114.34  0.3904       8.61       8.00     7.6  10.000
 XorBinaryFuseFilter8-Prefetched   83.05    0.00    7.06    7.08    7.09    7.13    7.11  104.33  0.3884       9.02       8.01    12.6  10.000
Sort time: 81 ns/key
M1
❯ ./bulk-insert-and-query.exe 10000000 0,98,100                                                              find    find    find    find    find  1*add+                       optimal  wasted million                                     add  remove      0%     25%     50%     75%    100%  3*find      ε%  bits/item  bits/item  space%    keys                            Xor8   76.09    0.00   10.97   10.12   10.11   10.05   10.03  106.87  0.3911       9.84       8.00    23.0  10.000XorBinaryFuseFilter8-4WisePrefetch   59.75    0.00   10.02    9.93    9.79    9.97    9.67   89.39  0.3930       8.61       7.99     7.8  10.000 XorBinaryFuseFilter8-Prefetched   53.00    0.00    9.02    8.79    8.77    8.71    8.80   79.45  0.3902       9.02       8.00    12.7  10.000Sort time: 60 ns/key
